Flash Cache: Reducing Bias in Radiance Cache Based Inverse Rendering

State-of-the-art techniques for 3D reconstruction are largely based on volumetric scene representations, which require sampling multiple points to compute the color arriving along a ray. Using these representations for more general inverse rendering -- reconstructing geometry, materials, and lighting from observed images -- is challenging because recursively path-tracing such volumetric representations is expensive. Recent works alleviate this issue through the use of radiance caches: data structures that store the steady-state, infinite-bounce radiance arriving at any point from any direction. However, these solutions rely on approximations that introduce bias into the renderings and, more importantly, into the gradients used for optimization. We present a method that avoids these approximations while remaining computationally efficient. In particular, we leverage two techniques to reduce variance for unbiased estimators of the rendering equation: (1) an occlusion-aware importance sampler for incoming illumination and (2) a fast cache architecture that can be used as a control variate for the radiance from a high-quality, but more expensive, volumetric cache. We show that by removing these biases our approach improves the generality of radiance cache based inverse rendering, as well as increasing quality in the presence of challenging light transport effects such as specular reflections.

==> figures/rebuttal_bias.tex <==
\begin{figure}[t!]
    \centering
    %\includegraphics[draft=\isdraft,width=3in,height=4in]{figures/fig1.jpg}
    % \footnotesize
    %\begin{tabular}{@{}c@{\hspace{2pt}}c@{}}
    %     \includegraphics[trim={0 11cm 0 5cm},clip,width=0.47\linewidth]{figures/rebuttal/thinstructure_tensoir.jpg} &
    %     \includegraphics[trim={0 11cm 0 5cm},clip,width=0.47\linewidth]{figures/rebuttal/thinstructure_ours.jpg}
    %\end{tabular}\vspace{0pt}
    \begin{tabular}{@{}c@{\hspace{2pt}}c@{}}
         \includegraphics[trim={0 5cm 0 7cm},clip,width=0.47\linewidth]{figures/rebuttal/indirect_ours_2.png} &
         \includegraphics[trim={0 1cm 0 12cm},width=0.47\linewidth]{figures/rebuttal/indirect_invrender.PNG}

    \end{tabular}\vspace{-8pt}
    % \vspace{3pt}
    \caption{\label{fig:bias}%
    %\textbf{Row 1:} Our method (right) captures thin structures better than TensoIR (left). 
    Our method (left) more accurately models indirect illumination, e.g. reflections, than InvRender (right).
    }\vspace{-6pt}
    %\caption{\textbf{Structured light can overcome depth ambiguities.} Replace with a compelling result comparison. \matt{Need to come up with teaser that better highlights the key contributions of this work, not the method.  Should be flashy.}}
\end{figure}

==> figures/rebuttal_hotdog.tex <==
% \begin{table}[t]
% \centering
% \caption{Comparisons to NeX.}
% \small
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{%
% @{}%
% l@{\hspace{0.8\tabcolsep}}%
% c@{\hspace{0.4\tabcolsep}}%
% c@{\hspace{0.4\tabcolsep}}%
% c@{\hspace{0.8\tabcolsep}}%
% c@{\hspace{0.4\tabcolsep}}%
% c@{\hspace{0.4\tabcolsep}}%
% c@{\hspace{0.8\tabcolsep}}%
% c@{\hspace{0.4\tabcolsep}}%
% c@{\hspace{0.4\tabcolsep}}%
% c@{}%
% }
% \toprule
% \multirow{2}{*}[-0.5ex]{Method}
% & \multicolumn{3}{c}{Stanford}
% & \multicolumn{3}{c}{Undistorted Real FF}
% & \multicolumn{3}{c}{Shiny} \\
% \cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule{8-10}
% & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$
% & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$
% & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
% \midrule
% NeX &&&&&&&&& \\
% Ours &&&&&&&&& \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:nex}
% \end{table}


\begin{table}[t]
\centering
\caption{Equal training time comparison on the \textit{Hotdog} scene}
\small
\resizebox{\linewidth}{!}{
\begin{tabular}{%
@{}%
l@{\hspace{0.8\tabcolsep}}%
c@{\hspace{0.4\tabcolsep}}%
c@{\hspace{0.4\tabcolsep}}%
c@{\hspace{0.8\tabcolsep}}%
c@{\hspace{0.4\tabcolsep}}%
c@{\hspace{0.4\tabcolsep}}%
c@{\hspace{0.8\tabcolsep}}%
c@{\hspace{0.4\tabcolsep}}%
c@{\hspace{0.4\tabcolsep}}%
c@{}%
}
\toprule
\multirow{2}{*}[-0.5ex]{Metric}
& \multicolumn{3}{c}{Albedo}
& \multicolumn{3}{c}{NVS}
& \multicolumn{3}{c}{Relighting} \\
\cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule{8-10}
& PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$
& PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$
& PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
\midrule
TensoIR
 & \bf 30.370 & 0.947 & 0.093
 & 36.820 & \bf 0.976 & \bf 0.045
 & 27.927 & 0.933 & 0.115
\\
Ours
 & 29.617 & \bf 0.957 & \bf 0.092
 & \bf 37.393 & 0.964 & 0.087
 & \bf 28.830 & \bf 0.941 & \bf 0.101
\\
\bottomrule
\end{tabular}
}
\label{tab:hotdog}
\vspace{-10pt}
\end{table}



==> figures/rebuttal_specular.tex <==
\begin{figure}[t!]
    \centering
    %\includegraphics[draft=\isdraft,width=3in,height=4in]{figures/fig1.jpg}
    % \footnotesize
    \begin{tabular}{@{}c@{\hspace{2pt}}c@{}}
         \includegraphics[trim={0cm 15cm 0cm 0cm},clip,width=0.47\linewidth]{figures/rebuttal/geometry_ours.png} &
         \includegraphics[trim={3.0cm 8.2cm 3.0cm 0cm},clip,width=0.3\linewidth]{figures/rebuttal/geometry_nero.PNG}
    \end{tabular}\vspace{-5.1pt}
    \begin{tabular}{@{}c@{\hspace{2pt}}c@{}}
         \includegraphics[trim={0cm 6cm 0cm 13cm},clip,width=0.47\linewidth]{figures/rebuttal/color_ours.png} &
         \includegraphics[trim={3.0cm 4cm 3.0cm 6cm},clip,width=0.3\linewidth]{figures/rebuttal/geometry_nero.PNG}
    \end{tabular}\vspace{-7pt}
    % \vspace{3pt}
    \caption{\label{fig:bias}%
    (Left) Our method recovers the geometry and appearance of a specular object. (Right) NeRO fails to recover several thin structures, e.g. hairs on the top of the horse's head and mane.
    }\vspace{-17pt}
    %\caption{\textbf{Structured light can overcome depth ambiguities.} Replace with a compelling result comparison. \matt{Need to come up with teaser that better highlights the key contributions of this work, not the method.  Should be flashy.}}
\end{figure}

==> figures/results_old.tex <==
\begin{figure*}[t]
\footnotesize

\mpage{1.0}{%

    \mpage{0.32}{%
        Ground Truth Albedo
    }\hspace{-1mm}\hfill%
    \mpage{0.32}{%
        Our Albedo
    }\hspace{-1mm}\hfill%
    \mpage{0.32}{%
         TensoIR Albedo
    }\hspace{-1mm}\hfill%

    \mpage{0.32}{%
        \adjincludegraphics[width=\linewidth]{figures/results_jpeg/hotdog_albedo_gt.jpg}\\[0.2mm]%
    }\hspace{-1mm}\hfill%
    \mpage{0.32}{%
        \adjincludegraphics[width=\linewidth]{figures/results_jpeg/hotdog_albedo_ours.jpg}\\[0.2mm]%
    }\hspace{-1mm}\hfill%
    \mpage{0.32}{%
        \adjincludegraphics[width=\linewidth]{figures/results_jpeg/hotdog_albedo_tensoir.jpg}\\[0.2mm]%
    }\hspace{-1mm}\hfill%

    \mpage{0.32}{%
        Ground Truth Relit
    }\hspace{-1mm}\hfill%
    \mpage{0.32}{%
        Our Relit
    }\hspace{-1mm}\hfill%
    \mpage{0.32}{%
         TensoIR Relit
    }\hspace{-1mm}\hfill%

    \mpage{0.32}{%
        \adjincludegraphics[width=\linewidth]{figures/results_jpeg/hotdog_relight_gt.jpg}\\[0.2mm]%
    }\hspace{-1mm}\hfill%
    \mpage{0.32}{%
        \adjincludegraphics[width=\linewidth]{figures/results_jpeg/hotdog_relight_ours.jpg}\\[0.2mm]%
    }\hspace{-1mm}\hfill%
    \mpage{0.32}{%
        \adjincludegraphics[width=\linewidth]{figures/results_jpeg/hotdog_relight_tensoir.jpg}\\[0.2mm]%
    }\hspace{-1mm}\hfill%

    \mpage{0.32}{%
        Ground Truth Albedo
    }\hspace{-1mm}\hfill%
    \mpage{0.32}{%
        Our Albedo
    }\hspace{-1mm}\hfill%
    \mpage{0.32}{%
         TensoIR Albedo
    }\hspace{-1mm}\hfill%

    \mpage{0.32}{%
        \adjincludegraphics[width=\linewidth]{figures/results_jpeg/ficus_albedo_gt.jpg}\\[0.2mm]%
    }\hspace{-1mm}\hfill%
    \mpage{0.32}{%
        \adjincludegraphics[width=\linewidth]{figures/results_jpeg/ficus_albedo_ours.jpg}\\[0.2mm]%
    }\hspace{-1mm}\hfill%
    \mpage{0.32}{%
        \adjincludegraphics[width=\linewidth]{figures/results_jpeg/ficus_albedo_tensoir.jpg}\\[0.2mm]%
    }\hspace{-1mm}\hfill%

    \mpage{0.32}{%
        Ground Truth Relit
    }\hspace{-1mm}\hfill%
    \mpage{0.32}{%
        Our Relit
    }\hspace{-1mm}\hfill%
    \mpage{0.32}{%
         TensoIR Relit
    }\hspace{-1mm}\hfill%

    \mpage{0.32}{%
        \adjincludegraphics[width=\linewidth]{figures/results_jpeg/ficus_relight_gt.jpg}\\[0.2mm]%
    }\hspace{-1mm}\hfill%
    \mpage{0.32}{%
        \adjincludegraphics[width=\linewidth]{figures/results_jpeg/ficus_relight_ours.jpg}\\[0.2mm]%
    }\hspace{-1mm}\hfill%
    \mpage{0.32}{%
        \adjincludegraphics[width=\linewidth]{figures/results_jpeg/ficus_relight_tensoir.jpg}\\[0.2mm]%
    }\hspace{-1mm}\hfill%
    
}
\caption{%
\TODO{Results}
}%
%
\label{fig:qual}
\vspace{-5mm}
\end{figure*}


==> figures/supptab1_smoothness.tex <==
\begin{table*}[t]
%\begin{SCtable}[75]
\centering
\caption{
\textbf{Smoothness Ablations}
}
\vspace{-0.1in}
\begin{tabular}{l c@{\,\,\,\,}c@{\,\,\,\,}c}
    \toprule
    Method & NVS PSNR$\uparrow$ & Albedo PSNR$\uparrow$ & MAE$\downarrow$ \\ \hline

    \phantom{(a)} Ours & 34.915 & 30.345 & 3.355  \\
    \bottomrule
\end{tabular}
\label{tab:smoothness}
%\end{SCtable}
\end{table*}
